Quantum-assisted associative adversarial network: Applying quantum annealing in deep learning

We present an algorithm for learning a latent variable generative model via generative adversarial learning where the canonical uniform noise input is replaced by samples from a graphical model. This graphical model is learned by a Boltzmann machine which learns low-dimensional feature representation of data extracted by the discriminator. A quantum annealer, the D-Wave 2000Q, is used to sample from this model. This algorithm joins a growing family of algorithms that use a quantum annealing subroutine in deep learning, and provides a framework to test the advantages of quantum-assisted learning in GANs. Fully connected, symmetric bipartite and Chimera graph topologies are compared on a reduced stochastically binarized MNIST dataset, for both classical and quantum annealing sampling methods. The quantum-assisted associative adversarial network successfully learns a generative model of the MNIST dataset for all topologies, and is also applied to the LSUN dataset bedrooms class for the Chimera topology. Evaluated using the Fr\'{e}chet inception distance and inception score, the quantum and classical versions of the algorithm are found to have equivalent performance for learning an implicit generative model of the MNIST dataset.

==> sections/notes/algorithms.tex <==
\begin{figure*}
\begin{minipage}{0.9\linewidth}
    \begin{algorithm}[H]
    \caption{\label{alg:qbm}Training a fully-visible and connected quantum Boltzmann machine with a quantum annealer, given \textbf{J} and \textbf{h} for one training epoch.}
        \begin{algorithmic}[1]
        \For{epochs}
        \State Sample batch of $n$ feature distribution samples from $\rho_f \rightarrow \boldsymbol{\psi} = \{\psi_1,\psi_2,...\psi_n\}$
        \State Map $\boldsymbol{\psi}$ to embedded space $\boldsymbol{\psi} \rightarrow \boldsymbol{\psi}'=\{\psi_1',\psi_2',...\psi_n'\}$
        \State Set $\textbf{J}$ and $\textbf{h}$
        \State Sample batch size \textit{n} from $\rho$ using annealer $\rho \rightarrow \{\phi_1, \phi_2, ..., \phi_n\}$
        \State  $\Delta J_{ij} = \eta[\langle z_i z_j \rangle_{\mathrm{data}} - \langle z_i z_j \rangle_{\mathrm{\rho}}]$ 
        \State $\Delta h_{i} = \eta[\langle z_i \rangle_{\mathrm{data}} - \langle z_i \rangle_{\mathrm{\rho}}]$ 
        \State $J_{ij} \leftarrow J_{ij} + \Delta J_{ij} $
        \State $h_i \leftarrow h_i + \Delta h_i$
        \EndFor
        \State \textbf{return} $\textbf{J}$ and $\textbf{h}$
        \end{algorithmic}
    \end{algorithm}
\end{minipage}
\caption{This algorithm is one epoch of training \gls{qbm} as outlined in Reference~\cite{benedetti2017quantum}. Sampling from the feature distribution $\rho_f$, equivalently labelled in Figure~\ref{fig:qaaan}, is written $\rho_f \rightarrow \boldsymbol{\psi}$ giving set $\boldsymbol{\psi}$ containing samples $\psi_n$. $\boldsymbol{\psi}'$ is set of samples in embedded space, there is a many-to-one mapping between  $\boldsymbol{\psi}'$ and $\boldsymbol{\psi}$. $\rho$ is the \gls{qbm} model, and $\textbf{h}$ and $\textbf{J}$ are the set of local fields and couplings between qubits, respectively. $\eta$ is the learning rate and is typically of the order $10^{-3}$.}
\end{figure*}

==> sections/notes/disc.tex <==

\section{Results \& Discussion}

Three topologies for the latent space were evaluated for performance on learning a reduced, stochastically binarized version of MNIST. 

Sparse, restricted and complete latent space topologies were implemented using classical MCMC sampling methods from a Boltzmann machine. A set of 64 randomly generated images is shown in Figure~\ref{fig:mnist_classical} from the classical sparse latent space topology. A sparse topology latent space algorithm was implemented using sampling from the D-Wave 2000Q and the generated images shown in Figure~\ref{fig:mnist_quantum}.

\begin{figure}[t]
 \subfloat[\label{fig:mnist_classical}]{%
   \includegraphics[width=0.35\textwidth]{figs/mnist_classical.png}
 }
 \hfill
 \subfloat[\label{fig:mnist_quantum}]{%
   \includegraphics[width=0.35\textwidth]{figs/mnist_gen_quantum.png}
 }
 \caption{Example MNIST characters generated by quantum and classical associative adversarial network architectures.}
 \label{fig:digits}
\end{figure}

These architectures were evaluated using the \gls{is} and \gls{fid}.

% https://arxiv.org/pdf/1801.01973.pdf do estimator 10x with N=5000 to find inception score

The Inception Score, Equation~\ref{eq:inception_score}, attempts to quantify realism of images generated by a model. For a given image, $p(y | x)$ should be dominated by one value of $y$, indicating a high probability that an image is representative of a class. Secondly, over the whole set there should be a uniform distribution of classes, indicating diversity of the distribution. This is expressed

\begin{equation}
    \mathrm{IS} = \exp( \EX_{x\sim\rho_\mathrm{D}} \mathrm{D}_\mathrm{KL}(p(y | x) || p(y))).
    \label{eq:inception_score}
\end{equation}

The first criterion is satisfied by requiring that image-wise class distributions should have low entropy. The second criterion implies that the entropy of the overall distribution should be high. The method is to calculate the KL distance between these two distributions: A high value indicates that both the $p(y|x)$ is distributed over one class and $p(y)$ is distributed over many classes. When averaged over all samples this score gives a good indication of the performance of the network. 

The \gls{fid} measures the similarity between features extracted by an inception network from the dataset $X$ and the generated data $G$. The distribution of the features are modelled as a mutlivariate Gaussian. Lower FID values mean the features extracted from the generated images are closer those for the real images. In Equation~\ref{eq:frechet_inception_distance}, $\mu$ are the means of the activations of an interim layer of the inception network and $\Sigma$ are the covariance matrices of these activations. The inception network used to evaluate both of these scores was trained to an accuracy of ~95\%.
% [200/200], Step [200/600], Loss: 1.5358, Accuracy: 95.1000%


\begin{equation}
    \mathrm{FID}(X, G) = ||\mu_X - \mu_G||^2_2 + \Tr(\Sigma_X + \Sigma_G - 2\sqrt{\Sigma_X \Sigma_G})
    \label{eq:frechet_inception_distance}
\end{equation}

The classical sparse network returned an FID of $\sim22$
The quantum sparse network captured an FID of $\sim22$ also and an inception distance of $\sim6$.  

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figs/topology_comparison_quantum.png}
    \caption{Comparison of the convergence of different graphical topologies trained using samples from a quantum annealers on a reduced stochastically binarized MNIST dataset.}
    \label{fig:topology_comparison_quantum}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figs/topology_comparison_classical.png}
    \caption{Comparison of different graphical topologies trained using MCMC sampling on a reduced stochastically binarized MNIST dataset.}
    \label{fig:topology_comparison_classical}
\end{figure}




\subsubsection*{Discussion}

In tests we unsurprisingly found a direct correlation between the number of latent space nodes and the quality of the images generated. 

What the results mean

Though these values are not comparable to state-of-the-art \gls{gan} architectures and are on a simple MNIST implementation, they serve the purpose of highlighting that the inclusion of a rudimentary quantum device is not detrimental to the performance of this scalable algorithm.

As expected there was a notable gain in performance when using the pause comparable to that observed for optimisation problems \cite{marshall2018power}. Here, though the only goal was to highlight the performance gains, we assume the same underlying physics: Relaxation of the system after excitations occur after the minimum gap. 

Though it is trivial to demonstrate a correlation between the connectivity of a graphical model and the quality of the learned model, Figure~\ref{fig:topology_comparison_classical}, it is not immediately clear that the benefits of increasing the complexity of the latent space can be detected easily in deep learning frameworks, such as the quantum-assisted Helmholtz machine \cite{benedetti2018quantumqahm} and those looking to exploit quantum models \cite{khoshaman2018quantum}. 

We found indistinguishable performance for classical and quantum implementations, indicating that even the limitations of near-term devices are not detrimental to the implementation of this framework. Secondly, we have demonstrated the framework on the larger, more complex dataset LSUN bedrooms, Figure~\ref{fig:lsun}. This shows that the algorithm can be scaled. 

It is not possible to detect the change in performance when using the pause or when changing topologies, indicating that any deep learning frameworks looking to exploit quantum hardware supported training in the latent spaces need to truly benefit from this application and not iron out any potential benefits with backpropagation. 




==> sections/topologies_pausing.tex <==







